Variation in the Stellar Mass Function Along Stellar Streams

Stellar streams are the inevitable end product of star cluster evolution, with the properties of a given stream being related to its progenitor. We consider how the dynamical history of a progenitor cluster, as traced by the evolution of its stellar mass function, is reflected in the resultant stream. We generate model streams by evolving star clusters with a range of initial half-mass relaxation times and dissolution times via direct N-body simulations. Stellar streams that dissolve quickly show no variation in the stellar mass function along the stream. Variation is, however, observed along streams with progenitor clusters that dissolve after several relaxation times. The mass function at the edges of a stream is approximately primordial as it is populated by the first stars to escape the cluster before segregation occurs. Moving inwards the mass function steepens as the intermediate parts of the stream consist of mostly low-mass stars that escaped the cluster after some segregation has occurred. The centre of the stream is then marked by a flatter mass function, as the region is dominated by high-mass stars that quickly segregated to the progenitor cluster's centre and were the last stars to become unbound. We further find that the maximum slope of the mass function along the stream and the rate at which it decreases with distance from the dissolved progenitor serve as proxies for the dynamical state reached by the progenitor cluster before dissolution; this may be able to be applied to observed streams with near-future observations.

==> notes.tex <==
%% Define notes using todonotes package

\usepackage{xparse}
\usepackage{ifthen}

\makeatletter
% Set this option to 1 for notes, 0 to disable notes
\newcommand{\@todonotes@enable}{1}
% Set this option to 1 for inline comments, 0 for margin comments
\newcommand{\@todonotes@inline}{1}
\makeatother
\input{notes.tex}
\newcommand{\jw}[1]{\note[red]{JW: #1}}
\newcommand{\jb}[1]{\note[darkblue][vlightblue]{JB: #1}}

% Increase margins for margin comments
\ifthenelse{\@todonotes@enable=1 \AND \@todonotes@inline=0}{
\paperwidth=\dimexpr\paperwidth + 6cm\relax
%\textwidth=\dimexpr \textwidth - 6cm\relax
\oddsidemargin=\dimexpr\oddsidemargin + 3cm\relax
\evensidemargin=\dimexpr\evensidemargin + 3cm\relax
\marginparwidth=\dimexpr \marginparwidth + 2.5cm\relax}{}

\ifthenelse{\@todonotes@enable=1}
  {\usepackage[textwidth=\dimexpr\evensidemargin + 2.25cm]{todonotes}}
  {\usepackage[disable]{todonotes}}

% Colors for comment boxes
\definecolor{gold}{RGB}{255,215,0}
\definecolor{salmon}{rgb}{0.95,0.5,0.25}
\definecolor{darkgreen}{rgb}{0.0, 0.5, 0.0}
\definecolor{darkblue}{rgb}{0.0, 0., 0.7}
\definecolor{vlightblue}{rgb}{0.68,0.84,0.9}
\definecolor{purple}{rgb}{0.7, 0., 0.7}
\definecolor{lavender}{rgb}{0.9, 0.9, 0.98}

\newcommand{\@todonotes@loaded}{0}
\@ifpackageloaded{todonotes}
  {\renewcommand{\@todonotes@loaded}{1}}
  {\renewcommand{\@todonotes@loaded}{0}}
% Deal with inline: hack
\ifthenelse{\@todonotes@inline=0}
  {\renewcommand{\@todonotes@loaded}{1}}
  {\renewcommand{\@todonotes@loaded}{0}}
\@ifpackagewith{todonotes}{disable}
  {\renewcommand{\@todonotes@loaded}{0}}
  {}

% Increase margins for margin comments
%\ifthenelse{\@todonotes@loaded=1}{
%\textwidth=\dimexpr \textwidth - 6cm\relax
%\oddsidemargin=\dimexpr\oddsidemargin + 3cm\relax
%\evensidemargin=\dimexpr\evensidemargin + 3cm\relax
%\marginparwidth=\dimexpr \marginparwidth + 2.5cm\relax}{}

\ifthenelse{\@todonotes@inline=1}{
\NewDocumentCommand{\note}{O{black} O{gold} m}{\todo[inline,backgroundcolor={#2},linecolor={#2},bordercolor={#1}]{{\protect\footnotesize #3}}}}
{\NewDocumentCommand{\note}{O{black} O{gold} m}{\todo[backgroundcolor={#2},linecolor={#2},bordercolor={#1}]{{\protect\footnotesize #3}}}}
\makeatother
